Component based model order reduction with mortar tied contact for nonlinear quasi-static mechanical problems

In this work, we present a model order reduction technique for nonlinear structures assembled from components.The reduced order model is constructed by reducing the substructures with proper orthogonal decomposition and connecting them by a mortar-tied contact formulation. The snapshots for the substructure projection matrices are computed on the substructure level by the proper orthogonal decomposition (POD) method. The snapshots are computed using a random sampling procedure based on a parametrization of boundary conditions. To reduce the computational effort of the snapshot computation full-order simulations of the substructures are only computed when the error of the reduced solution is above a threshold. In numerical examples, we show the accuracy and efficiency of the method for nonlinear problems involving material and geometric nonlinearity as well as non-matching meshes. We are able to predict solutions of systems that we did not compute in our snapshots.

==> sections/section1.tex <==
\section{A super nice section}
\label{sec:1}

This section is really great! And there is also awesome Fig.~\ref{fig:1}.
\begin{figure}[htbp]
  \centering
  \includegraphics{./images/drawing}
  \caption{Awesome figure}
  \label{fig:1}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> sections/section2.tex <==
\section{Yet another super nice section}
\label{sec:2}

But this section here is even better! Here we have additionally the
following subsection.

\subsection{A super nice subsection}
\label{sec:2-1}

Furthermore, we even refer to the outstanding
reference \cite{BrepolsWulfinghoffEtAl2017}. Moreover, we refer to Appendix~\ref{sec:3-1}. 




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 

